Can LLM Generate Culturally Relevant Commonsense QA Data? Case Study in Indonesian and Sundanese

Large Language Models (LLMs) are increasingly being used to generate synthetic data for training and evaluating models. However, it is unclear whether they can generate a good quality of question answering (QA) dataset that incorporates knowledge and cultural nuance embedded in a language, especially for low-resource languages. In this study, we investigate the effectiveness of using LLMs in generating culturally relevant commonsense QA datasets for Indonesian and Sundanese languages. To do so, we create datasets for these languages using various methods involving both LLMs and human annotators, resulting in ~4.5K questions per language (~9K in total), making our dataset the largest of its kind. Our experiments show that automatic data adaptation from an existing English dataset is less effective for Sundanese. Interestingly, using the direct generation method on the target language, GPT-4 Turbo can generate questions with adequate general knowledge in both languages, albeit not as culturally 'deep' as humans. We also observe a higher occurrence of fluency errors in the Sundanese dataset, highlighting the discrepancy between medium- and lower-resource languages.

==> latex/tables/answer_acc_ind_sun.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lcc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Status}}} & \multicolumn{2}{c}{\textbf{\% of correct answer}}                                    \\ \cmidrule(l){2-3} 
\multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{\textbf{\texttt{ind}}} & \multicolumn{1}{c}{\textbf{\texttt{sun}}} \\ \midrule
\textsc{LLM\_Adapt}                & 92.41\%                            & N/A                     \\
\textsc{LLM\_Gen}                 & \textbf{95.00\%}                            & \textbf{90.67\%}                     \\ \bottomrule
\end{tabular}
\caption{Answer generation accuracy of \textsc{LLM\_Adapt} and \textsc{LLM\_Gen}.}
\label{tab:answer_acc_ind_sun}
\end{table}

==> latex/tables/benchmark_raw.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}llllrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Test Size}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model Type}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model Name}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Size}}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} \\ \cmidrule(l){6-7} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{ind}} &
  \multicolumn{1}{c}{\textbf{sun}} \\ \midrule
\multirow{8}{*}{adapt\_csqa} &
  \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}158 (ind)\\ 158 (sun)\end{tabular}} &
  \multirow{5}{*}{Open Source} &
  BLOOMZ &
  7b &
  \textbf{58.02} &
  31.22 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  \multirow{2}{*}{LLaMA-2} &
  7b &
  50.00 &
  30.59 \\
 &
   &
   &
   &
  13b &
  50.00 &
  33.54 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  PolyLM &
  13b &
  30.06 &
  22.57 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  SeaLLM &
  7b &
  51.05 &
  \textbf{35.65} \\ \cmidrule(l){3-7} 
 &
   &
  \multirow{3}{*}{Proprietary} &
  GPT-3.5 &
  N/A &
  64.56 &
  43.88 \\
 &
   &
   &
  GPT-4 &
  N/A &
  72.36 &
  54.43 \\
 &
   &
   &
  GPT-4-turbo &
  N/A &
  \textbf{76.79} &
  \textbf{65.82} \\ \midrule
\multirow{8}{*}{manual\_csqa} &
  \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}1,498 (ind)\\ 1,499 (sun)\end{tabular}} &
  \multirow{5}{*}{Open Source} &
  BLOOMZ &
  7b &
  \textbf{62.15} &
  37.56 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  \multirow{2}{*}{LLaMA-2} &
  7b &
  44.66 &
  34.80 \\
 &
   &
   &
   &
  13b &
  50.58 &
  34.76 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  PolyLM &
  13b &
  31.62 &
  24.17 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  SeaLLM &
  7b &
  58.28 &
  \textbf{41.47} \\ \cmidrule(l){3-7} 
 &
   &
  \multirow{3}{*}{Proprietary} &
  GPT-3.5 &
  N/A &
  79.39 &
  55.97 \\
 &
   &
   &
  GPT-4 &
  N/A &
  \textbf{90.97} &
  71.18 \\
 &
   &
   &
  GPT-4-turbo &
  N/A &
  \textbf{90.97} &
  \textbf{81.37} \\ \midrule
\multirow{8}{*}{auto\_csqa} &
  \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}1,062 (ind)\\ 1,291 (sun)\end{tabular}} &
  \multirow{5}{*}{Open Source} &
  BLOOMZ &
  7b &
  76.46 &
  \textbf{49.99} \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  \multirow{2}{*}{LLaMA-2} &
  7b &
  70.12 &
  46.45 \\
 &
   &
   &
   &
  13b &
  76.24 &
  50.86 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  PolyLM &
  13b &
  39.27 &
  23.52 \\ \cdashline{4-7} \addlinespace[0.5ex]
 &
   &
   &
  SeaLLM &
  7b &
  \textbf{79.25} &
  49.86 \\ \cmidrule(l){3-7} 
 &
   &
  \multirow{3}{*}{Proprietary} &
  GPT-3.5 &
  N/A &
  87.85 &
  70.57 \\
 &
   &
   &
  GPT-4 &
  N/A &
  93.35 &
  79.63 \\
 &
   &
   &
  GPT-4-turbo &
  N/A &
  \textbf{94.29} &
  \textbf{85.36} \\ \bottomrule
\end{tabular}
\caption{Benchmark result (raw -- before manual evaluation).}
\label{tab:benchmark_raw}
\end{table*}

==> latex/tables/concept_wrong_ind.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lr@{}}
\toprule
\textbf{Wrong Reason}        & \textbf{Num} \\ \midrule
Translation error            & 4            \\
Sentence structure error     & 1            \\
Typo or capitalization error & 2            \\ \bottomrule
\end{tabular}
\caption{Summary of errors of English to Indonesian concept adaptation.}
\label{tab:errors_ind}
\end{table}

==> latex/tables/concept_wrong_sun.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lr@{}}
\toprule
\textbf{Wrong Reason}        & \textbf{Num} \\ \midrule
Translation error            & 28           \\
Sentence structure error     & 1            \\
Typo or capitalization error & 4            \\
Word form error              & 3            \\ \bottomrule
\end{tabular}
\caption{Summary of errors of Indonesian to Sundanese concept adaptation.}
\label{tab:errors_sun}
\end{table}

==> latex/tables/worksheet_field.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Field}} & \multicolumn{1}{c}{\textbf{Description}}                                                                  \\ \midrule
ID                                 & This column contains the ID of each data.                                                                 \\ \midrule
Category                           & This column contains the overarching category of the data.                                                \\ \midrule
Question Concept                   & This column contains concepts from categories that need to be used in creating questions.                 \\ \midrule
Question                           & This column is used to write commonsense questions that contain the given concept and match the category. \\ \midrule
Choices &
  \begin{tabular}[c]{@{}l@{}}This column is used to write 5 choices for the questions given. Of the 5 choices given, the annotator needs to\\ ensure there is 1 correct answer and 1 distractor. Distractor is an answer that could potentially be considered\\ the correct answer.\end{tabular} \\ \midrule
Answer                             & This column only needs to be filled in when the row contains the correct answer.                          \\ \midrule
Distractor                         & This column only needs to be filled in when the row contains the distractor.                              \\ \bottomrule
\end{tabular}
\caption{The detailed criteria and field for creating commonsense QA data.}
\label{tab:worksheet_field}
\end{table*}
